GWTC-5.0: Population Properties of Merging Compact Binaries

We present the population properties of merging compact binaries inferred using 267 mergers from the cumulative Gravitational-Wave Transient Catalog 5.0. As this data set contains no new sources with a neutron star, we primarily focus on the properties of the binary black hole mergers. We infer the merger rate of binary black holes with component masses between $2.5\,\mathrm{M}_\odot $ and $200\,\mathrm{M}_\odot $ to be $27.5\text{--} 49.4 \, \mathrm{Gpc}^{-3}\,\mathrm{yr}^{-1}$ (all intervals at $90\%$ credible levels) at redshift $z = 0.2$. We find evidence for a subpopulation of binary black hole mergers that host a rapidly spinning black hole (dimensionless spins $\chi \sim 0.7$), consistent with signatures of hierarchical mergers. We find that these occur at two mass scales, the first at primary masses $\sim 10$--$20\,\mathrm{M}_\odot $ and the second above $\sim 45\,\mathrm{M}_\odot $, and we estimate their total rate at $z=0.2$ to be $0.2\text{--} 3.11 \, {\rm Gpc}^{-3} {\rm yr}^{-1}$. We infer that, above $40\,\mathrm{M}_\odot $, the mass distribution of the less massive (secondary) black hole declines more steeply than that of the more massive (primary) one. This is consistent with a flatter mass-ratio distribution and indicates the prevalence of unequal-mass binaries with large primary masses. We find evidence for two features in the black hole mass spectrum: a peak around $10\,\mathrm{M}_\odot $ and a change of slope at around $35\,\mathrm{M}_\odot $. Black holes of $\sim 35\,\mathrm{M}_\odot $ pair preferentially with companions of similar mass. Additionally, we find that the effective inspiral spin distribution of binary black holes is asymmetric about zero, based on which we infer that at least $9 \%$ of mergers occur in channels with some preference for spin-orbit alignment. We find evidence that...

==> macros_from_json.tex <==
\makeatletter%
\newcommand\HierarchicalMacros[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HierarchicalMacros@out{%
    \{%
      "rate\_uniform": \{%
        "median": 0.6,
        "5th percentile": 0.2,
        "95th percentile": 1.58,
        "error plus": 0.99,
        "error minus": 0.4%
      \},
      "uniform\_halfwidth": \{%
        "median": 0.37,
        "5th percentile": 0.26,
        "95th percentile": 0.5,
        "error plus": 0.13,
        "error minus": 0.11%
      \},
      "uniform\_mean": \{%
        "median": 0.04,
        "5th percentile": {-}0.06,
        "95th percentile": 0.13,
        "error plus": 0.09,
        "error minus": 0.09%
      \},
      "gaussian\_mean": \{%
        "median": 0.03,
        "5th percentile": 0.01,
        "95th percentile": 0.04,
        "error plus": 0.01,
        "error minus": 0.01%
      \},
      "gaussian\_logstd": \{%
        "median": {-}1.24,
        "5th percentile": {-}1.33,
        "95th percentile": {-}1.15,
        "error plus": 0.09,
        "error minus": 0.09%
      \},
      "triple\_transistion\_uniform\_halfwidth\_low": \{%
        "median": 0.51,
        "5th percentile": 0.29,
        "95th percentile": 0.69,
        "error plus": 0.19,
        "error minus": 0.22%
      \},
      "triple\_transistion\_uniform\_mean\_low": \{%
        "median": 0.07,
        "5th percentile": {-}0.08,
        "95th percentile": 0.31,
        "error plus": 0.24,
        "error minus": 0.15%
      \},
      "triple\_transistion\_uniform\_halfwidth\_high": \{%
        "median": 0.47,
        "5th percentile": 0.24,
        "95th percentile": 0.62,
        "error plus": 0.16,
        "error minus": 0.23%
      \},
      "triple\_transistion\_uniform\_mean\_high": \{%
        "median": 0.07,
        "5th percentile": {-}0.05,
        "95th percentile": 0.31,
        "error plus": 0.24,
        "error minus": 0.13%
      \},
      "triple\_transistion\_gaussian\_mean": \{%
        "median": 0.02,
        "5th percentile": 0.01,
        "95th percentile": 0.04,
        "error plus": 0.01,
        "error minus": 0.01%
      \},
      "triple\_transistion\_gaussian\_logstd": \{%
        "median": {-}1.13,
        "5th percentile": {-}1.2,
        "95th percentile": {-}1.05,
        "error plus": 0.08,
        "error minus": 0.07%
      \},
      "triple\_transition\_m\_t\_low": \{%
        "median": 13.47,
        "5th percentile": 11.31,
        "95th percentile": 16.77,
        "error plus": 3.3,
        "error minus": 2.16%
      \},
      "triple\_transition\_m\_t\_mid": \{%
        "median": 20.24,
        "5th percentile": 18.1,
        "95th percentile": 34.02,
        "error plus": 13.78,
        "error minus": 2.14%
      \},
      "triple\_transition\_m\_t\_high": \{%
        "median": 41.62,
        "5th percentile": 34.55,
        "95th percentile": 54.19,
        "error plus": 12.58,
        "error minus": 7.06%
      \},
      "rates\_2g1g\_low\_mass": \{%
        "median": 1.22,
        "5th percentile": 0.37,
        "95th percentile": 2.68,
        "error plus": 1.46,
        "error minus": 0.85%
      \},
      "rates\_2g1g\_high\_mass": \{%
        "median": 0.38,
        "5th percentile": 0.1,
        "95th percentile": 0.73,
        "error plus": 0.36,
        "error minus": 0.28%
      \},
      "rates\_2g1g\_total": \{%
        "median": 1.63,
        "5th percentile": 0.67,
        "95th percentile": 3.11,
        "error plus": 1.48,
        "error minus": 0.96%
      \}%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{rate_uniform}=0%
      \let\HierarchicalMacros@out\HierarchicalMacros@I%
    \else%
      \ifnum\pdfstrcmp{#1}{uniform_halfwidth}=0%
      \let\HierarchicalMacros@out\HierarchicalMacros@II%
    \else%
      \ifnum\pdfstrcmp{#1}{uniform_mean}=0%
      \let\HierarchicalMacros@out\HierarchicalMacros@III%
    \else%
      \ifnum\pdfstrcmp{#1}{gaussian_mean}=0%
      \let\HierarchicalMacros@out\HierarchicalMacros@IV%
    \else%
      \ifnum\pdfstrcmp{#1}{gaussian_logstd}=0%
      \let\HierarchicalMacros@out\HierarchicalMacros@V%
    \else%
      \ifnum\pdfstrcmp{#1}{triple_transistion_uniform_halfwidth_low}=0%
      \let\HierarchicalMacros@out\HierarchicalMacros@VI%
    \else%
      \ifnum\pdfstrcmp{#1}{triple_transistion_uniform_mean_low}=0%
      \let\HierarchicalMacros@out\HierarchicalMacros@VII%
    \else%
      \ifnum\pdfstrcmp{#1}{triple_transistion_uniform_halfwidth_high}=0%
      \let\HierarchicalMacros@out\HierarchicalMacros@VIII%
    \else%
      \ifnum\pdfstrcmp{#1}{triple_transistion_uniform_mean_high}=0%
      \let\HierarchicalMacros@out\HierarchicalMacros@IX%
    \else%
      \ifnum\pdfstrcmp{#1}{triple_transistion_gaussian_mean}=0%
      \let\HierarchicalMacros@out\HierarchicalMacros@X%
    \else%
      \ifnum\pdfstrcmp{#1}{triple_transistion_gaussian_logstd}=0%
      \let\HierarchicalMacros@out\HierarchicalMacros@XI%
    \else%
      \ifnum\pdfstrcmp{#1}{triple_transition_m_t_low}=0%
      \let\HierarchicalMacros@out\HierarchicalMacros@XII%
    \else%
      \ifnum\pdfstrcmp{#1}{triple_transition_m_t_mid}=0%
      \let\HierarchicalMacros@out\HierarchicalMacros@XIII%
    \else%
      \ifnum\pdfstrcmp{#1}{triple_transition_m_t_high}=0%
      \let\HierarchicalMacros@out\HierarchicalMacros@XIV%
    \else%
      \ifnum\pdfstrcmp{#1}{rates_2g1g_low_mass}=0%
      \let\HierarchicalMacros@out\HierarchicalMacros@XV%
    \else%
      \ifnum\pdfstrcmp{#1}{rates_2g1g_high_mass}=0%
      \let\HierarchicalMacros@out\HierarchicalMacros@XVI%
    \else%
      \ifnum\pdfstrcmp{#1}{rates_2g1g_total}=0%
      \let\HierarchicalMacros@out\HierarchicalMacros@XVII%
    \else%
      \def\HierarchicalMacros@out{%
    ??}%
    \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
  \fi
  \HierarchicalMacros@out
}\newcommand\HierarchicalMacros@I[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HierarchicalMacros@I@out{%
    \{%
      "median": 0.6,
      "5th percentile": 0.2,
      "95th percentile": 1.58,
      "error plus": 0.99,
      "error minus": 0.4%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HierarchicalMacros@I@out{%
    0.6}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HierarchicalMacros@I@out{%
    0.2}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HierarchicalMacros@I@out{%
    1.58}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HierarchicalMacros@I@out{%
    0.99}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HierarchicalMacros@I@out{%
    0.4}%
    \else%
      \def\HierarchicalMacros@I@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HierarchicalMacros@I@out
}\newcommand\HierarchicalMacros@II[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HierarchicalMacros@II@out{%
    \{%
      "median": 0.37,
      "5th percentile": 0.26,
      "95th percentile": 0.5,
      "error plus": 0.13,
      "error minus": 0.11%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HierarchicalMacros@II@out{%
    0.37}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HierarchicalMacros@II@out{%
    0.26}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HierarchicalMacros@II@out{%
    0.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HierarchicalMacros@II@out{%
    0.13}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HierarchicalMacros@II@out{%
    0.11}%
    \else%
      \def\HierarchicalMacros@II@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HierarchicalMacros@II@out
}\newcommand\HierarchicalMacros@III[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HierarchicalMacros@III@out{%
    \{%
      "median": 0.04,
      "5th percentile": {-}0.06,
      "95th percentile": 0.13,
      "error plus": 0.09,
      "error minus": 0.09%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HierarchicalMacros@III@out{%
    0.04}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HierarchicalMacros@III@out{%
    {-}0.06}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HierarchicalMacros@III@out{%
    0.13}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HierarchicalMacros@III@out{%
    0.09}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HierarchicalMacros@III@out{%
    0.09}%
    \else%
      \def\HierarchicalMacros@III@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HierarchicalMacros@III@out
}\newcommand\HierarchicalMacros@IV[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HierarchicalMacros@IV@out{%
    \{%
      "median": 0.03,
      "5th percentile": 0.01,
      "95th percentile": 0.04,
      "error plus": 0.01,
      "error minus": 0.01%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HierarchicalMacros@IV@out{%
    0.03}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HierarchicalMacros@IV@out{%
    0.01}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HierarchicalMacros@IV@out{%
    0.04}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HierarchicalMacros@IV@out{%
    0.01}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HierarchicalMacros@IV@out{%
    0.01}%
    \else%
      \def\HierarchicalMacros@IV@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HierarchicalMacros@IV@out
}\newcommand\HierarchicalMacros@V[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HierarchicalMacros@V@out{%
    \{%
      "median": {-}1.24,
      "5th percentile": {-}1.33,
      "95th percentile": {-}1.15,
      "error plus": 0.09,
      "error minus": 0.09%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HierarchicalMacros@V@out{%
    {-}1.24}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HierarchicalMacros@V@out{%
    {-}1.33}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HierarchicalMacros@V@out{%
    {-}1.15}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HierarchicalMacros@V@out{%
    0.09}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HierarchicalMacros@V@out{%
    0.09}%
    \else%
      \def\HierarchicalMacros@V@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HierarchicalMacros@V@out
}\newcommand\HierarchicalMacros@VI[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HierarchicalMacros@VI@out{%
    \{%
      "median": 0.51,
      "5th percentile": 0.29,
      "95th percentile": 0.69,
      "error plus": 0.19,
      "error minus": 0.22%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HierarchicalMacros@VI@out{%
    0.51}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HierarchicalMacros@VI@out{%
    0.29}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HierarchicalMacros@VI@out{%
    0.69}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HierarchicalMacros@VI@out{%
    0.19}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HierarchicalMacros@VI@out{%
    0.22}%
    \else%
      \def\HierarchicalMacros@VI@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HierarchicalMacros@VI@out
}\newcommand\HierarchicalMacros@VII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HierarchicalMacros@VII@out{%
    \{%
      "median": 0.07,
      "5th percentile": {-}0.08,
      "95th percentile": 0.31,
      "error plus": 0.24,
      "error minus": 0.15%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HierarchicalMacros@VII@out{%
    0.07}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HierarchicalMacros@VII@out{%
    {-}0.08}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HierarchicalMacros@VII@out{%
    0.31}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HierarchicalMacros@VII@out{%
    0.24}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HierarchicalMacros@VII@out{%
    0.15}%
    \else%
      \def\HierarchicalMacros@VII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HierarchicalMacros@VII@out
}\newcommand\HierarchicalMacros@VIII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HierarchicalMacros@VIII@out{%
    \{%
      "median": 0.47,
      "5th percentile": 0.24,
      "95th percentile": 0.62,
      "error plus": 0.16,
      "error minus": 0.23%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HierarchicalMacros@VIII@out{%
    0.47}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HierarchicalMacros@VIII@out{%
    0.24}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HierarchicalMacros@VIII@out{%
    0.62}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HierarchicalMacros@VIII@out{%
    0.16}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HierarchicalMacros@VIII@out{%
    0.23}%
    \else%
      \def\HierarchicalMacros@VIII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HierarchicalMacros@VIII@out
}\newcommand\HierarchicalMacros@IX[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HierarchicalMacros@IX@out{%
    \{%
      "median": 0.07,
      "5th percentile": {-}0.05,
      "95th percentile": 0.31,
      "error plus": 0.24,
      "error minus": 0.13%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HierarchicalMacros@IX@out{%
    0.07}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HierarchicalMacros@IX@out{%
    {-}0.05}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HierarchicalMacros@IX@out{%
    0.31}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HierarchicalMacros@IX@out{%
    0.24}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HierarchicalMacros@IX@out{%
    0.13}%
    \else%
      \def\HierarchicalMacros@IX@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HierarchicalMacros@IX@out
}\newcommand\HierarchicalMacros@X[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HierarchicalMacros@X@out{%
    \{%
      "median": 0.02,
      "5th percentile": 0.01,
      "95th percentile": 0.04,
      "error plus": 0.01,
      "error minus": 0.01%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HierarchicalMacros@X@out{%
    0.02}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HierarchicalMacros@X@out{%
    0.01}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HierarchicalMacros@X@out{%
    0.04}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HierarchicalMacros@X@out{%
    0.01}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HierarchicalMacros@X@out{%
    0.01}%
    \else%
      \def\HierarchicalMacros@X@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HierarchicalMacros@X@out
}\newcommand\HierarchicalMacros@XI[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HierarchicalMacros@XI@out{%
    \{%
      "median": {-}1.13,
      "5th percentile": {-}1.2,
      "95th percentile": {-}1.05,
      "error plus": 0.08,
      "error minus": 0.07%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HierarchicalMacros@XI@out{%
    {-}1.13}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HierarchicalMacros@XI@out{%
    {-}1.2}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HierarchicalMacros@XI@out{%
    {-}1.05}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HierarchicalMacros@XI@out{%
    0.08}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HierarchicalMacros@XI@out{%
    0.07}%
    \else%
      \def\HierarchicalMacros@XI@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HierarchicalMacros@XI@out
}\newcommand\HierarchicalMacros@XII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HierarchicalMacros@XII@out{%
    \{%
      "median": 13.47,
      "5th percentile": 11.31,
      "95th percentile": 16.77,
      "error plus": 3.3,
      "error minus": 2.16%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HierarchicalMacros@XII@out{%
    13.47}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HierarchicalMacros@XII@out{%
    11.31}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HierarchicalMacros@XII@out{%
    16.77}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HierarchicalMacros@XII@out{%
    3.3}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HierarchicalMacros@XII@out{%
    2.16}%
    \else%
      \def\HierarchicalMacros@XII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HierarchicalMacros@XII@out
}\newcommand\HierarchicalMacros@XIII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HierarchicalMacros@XIII@out{%
    \{%
      "median": 20.24,
      "5th percentile": 18.1,
      "95th percentile": 34.02,
      "error plus": 13.78,
      "error minus": 2.14%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HierarchicalMacros@XIII@out{%
    20.24}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HierarchicalMacros@XIII@out{%
    18.1}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HierarchicalMacros@XIII@out{%
    34.02}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HierarchicalMacros@XIII@out{%
    13.78}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HierarchicalMacros@XIII@out{%
    2.14}%
    \else%
      \def\HierarchicalMacros@XIII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HierarchicalMacros@XIII@out
}\newcommand\HierarchicalMacros@XIV[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HierarchicalMacros@XIV@out{%
    \{%
      "median": 41.62,
      "5th percentile": 34.55,
      "95th percentile": 54.19,
      "error plus": 12.58,
      "error minus": 7.06%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HierarchicalMacros@XIV@out{%
    41.62}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HierarchicalMacros@XIV@out{%
    34.55}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HierarchicalMacros@XIV@out{%
    54.19}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HierarchicalMacros@XIV@out{%
    12.58}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HierarchicalMacros@XIV@out{%
    7.06}%
    \else%
      \def\HierarchicalMacros@XIV@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HierarchicalMacros@XIV@out
}\newcommand\HierarchicalMacros@XV[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HierarchicalMacros@XV@out{%
    \{%
      "median": 1.22,
      "5th percentile": 0.37,
      "95th percentile": 2.68,
      "error plus": 1.46,
      "error minus": 0.85%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HierarchicalMacros@XV@out{%
    1.22}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HierarchicalMacros@XV@out{%
    0.37}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HierarchicalMacros@XV@out{%
    2.68}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HierarchicalMacros@XV@out{%
    1.46}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HierarchicalMacros@XV@out{%
    0.85}%
    \else%
      \def\HierarchicalMacros@XV@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HierarchicalMacros@XV@out
}\newcommand\HierarchicalMacros@XVI[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HierarchicalMacros@XVI@out{%
    \{%
      "median": 0.38,
      "5th percentile": 0.1,
      "95th percentile": 0.73,
      "error plus": 0.36,
      "error minus": 0.28%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HierarchicalMacros@XVI@out{%
    0.38}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HierarchicalMacros@XVI@out{%
    0.1}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HierarchicalMacros@XVI@out{%
    0.73}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HierarchicalMacros@XVI@out{%
    0.36}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HierarchicalMacros@XVI@out{%
    0.28}%
    \else%
      \def\HierarchicalMacros@XVI@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HierarchicalMacros@XVI@out
}\newcommand\HierarchicalMacros@XVII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HierarchicalMacros@XVII@out{%
    \{%
      "median": 1.63,
      "5th percentile": 0.67,
      "95th percentile": 3.11,
      "error plus": 1.48,
      "error minus": 0.96%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HierarchicalMacros@XVII@out{%
    1.63}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HierarchicalMacros@XVII@out{%
    0.67}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HierarchicalMacros@XVII@out{%
    3.11}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HierarchicalMacros@XVII@out{%
    1.48}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HierarchicalMacros@XVII@out{%
    0.96}%
    \else%
      \def\HierarchicalMacros@XVII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HierarchicalMacros@XVII@out
}%
\makeatother%
\makeatletter%
\newcommand\HighMassEstimates[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HighMassEstimates@out{%
    \{%
      "m2\_13\_25Msun\_slope": \{%
        "median": {-}1.1,
        "5th percentile": {-}2.2,
        "95th percentile": {-}0.1,
        "error plus": 1.1,
        "error minus": 1.1%
      \},
      "m1\_40\_60Msun\_slope": \{%
        "median": {-}3.8,
        "5th percentile": {-}5.2,
        "95th percentile": {-}2.5,
        "error plus": 1.3,
        "error minus": 1.4%
      \},
      "m2\_40\_60Msun\_slope": \{%
        "median": {-}7.0,
        "5th percentile": {-}9.7,
        "95th percentile": {-}4.6,
        "error plus": 2.4,
        "error minus": 2.7%
      \},
      "40\_60Msun\_slope\_comparison": 97.7,
      "m1\_slope\_comparison": 94.8,
      "99.9th\_percentile\_m2\_dist": \{%
        "median": 57.9,
        "5th percentile": 47.7,
        "95th percentile": 96.6,
        "error plus": 38.7,
        "error minus": 10.2%
      \},
      "threesubpop\_onset\_of\_the\_third\_subpop": \{%
        "median": 46.6,
        "5th percentile": 39.9,
        "95th percentile": 58.2,
        "error plus": 11.6,
        "error minus": 6.7%
      \},
      "mean\_q\_of\_the\_third\_subpop": \{%
        "median": 0.6,
        "5th percentile": 0.2,
        "95th percentile": 0.9,
        "error plus": 0.3,
        "error minus": 0.5%
      \},
      "m2gap\_lower\_edge": \{%
        "median": 45.5,
        "5th percentile": 40.4,
        "95th percentile": 52.4,
        "error plus": 6.9,
        "error minus": 5.2%
      \}%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{m2_13_25Msun_slope}=0%
      \let\HighMassEstimates@out\HighMassEstimates@I%
    \else%
      \ifnum\pdfstrcmp{#1}{m1_40_60Msun_slope}=0%
      \let\HighMassEstimates@out\HighMassEstimates@II%
    \else%
      \ifnum\pdfstrcmp{#1}{m2_40_60Msun_slope}=0%
      \let\HighMassEstimates@out\HighMassEstimates@III%
    \else%
      \ifnum\pdfstrcmp{#1}{40_60Msun_slope_comparison}=0%
      \def\HighMassEstimates@out{%
    97.7}%
    \else%
      \ifnum\pdfstrcmp{#1}{m1_slope_comparison}=0%
      \def\HighMassEstimates@out{%
    94.8}%
    \else%
      \ifnum\pdfstrcmp{#1}{99.9th_percentile_m2_dist}=0%
      \let\HighMassEstimates@out\HighMassEstimates@IV%
    \else%
      \ifnum\pdfstrcmp{#1}{threesubpop_onset_of_the_third_subpop}=0%
      \let\HighMassEstimates@out\HighMassEstimates@V%
    \else%
      \ifnum\pdfstrcmp{#1}{mean_q_of_the_third_subpop}=0%
      \let\HighMassEstimates@out\HighMassEstimates@VI%
    \else%
      \ifnum\pdfstrcmp{#1}{m2gap_lower_edge}=0%
      \let\HighMassEstimates@out\HighMassEstimates@VII%
    \else%
      \def\HighMassEstimates@out{%
    ??}%
    \fi\fi\fi\fi\fi\fi\fi\fi\fi
  \fi
  \HighMassEstimates@out
}\newcommand\HighMassEstimates@I[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HighMassEstimates@I@out{%
    \{%
      "median": {-}1.1,
      "5th percentile": {-}2.2,
      "95th percentile": {-}0.1,
      "error plus": 1.1,
      "error minus": 1.1%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HighMassEstimates@I@out{%
    {-}1.1}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HighMassEstimates@I@out{%
    {-}2.2}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HighMassEstimates@I@out{%
    {-}0.1}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HighMassEstimates@I@out{%
    1.1}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HighMassEstimates@I@out{%
    1.1}%
    \else%
      \def\HighMassEstimates@I@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HighMassEstimates@I@out
}\newcommand\HighMassEstimates@II[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HighMassEstimates@II@out{%
    \{%
      "median": {-}3.8,
      "5th percentile": {-}5.2,
      "95th percentile": {-}2.5,
      "error plus": 1.3,
      "error minus": 1.4%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HighMassEstimates@II@out{%
    {-}3.8}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HighMassEstimates@II@out{%
    {-}5.2}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HighMassEstimates@II@out{%
    {-}2.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HighMassEstimates@II@out{%
    1.3}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HighMassEstimates@II@out{%
    1.4}%
    \else%
      \def\HighMassEstimates@II@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HighMassEstimates@II@out
}\newcommand\HighMassEstimates@III[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HighMassEstimates@III@out{%
    \{%
      "median": {-}7.0,
      "5th percentile": {-}9.7,
      "95th percentile": {-}4.6,
      "error plus": 2.4,
      "error minus": 2.7%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HighMassEstimates@III@out{%
    {-}7.0}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HighMassEstimates@III@out{%
    {-}9.7}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HighMassEstimates@III@out{%
    {-}4.6}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HighMassEstimates@III@out{%
    2.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HighMassEstimates@III@out{%
    2.7}%
    \else%
      \def\HighMassEstimates@III@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HighMassEstimates@III@out
}\newcommand\HighMassEstimates@IV[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HighMassEstimates@IV@out{%
    \{%
      "median": 57.9,
      "5th percentile": 47.7,
      "95th percentile": 96.6,
      "error plus": 38.7,
      "error minus": 10.2%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HighMassEstimates@IV@out{%
    57.9}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HighMassEstimates@IV@out{%
    47.7}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HighMassEstimates@IV@out{%
    96.6}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HighMassEstimates@IV@out{%
    38.7}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HighMassEstimates@IV@out{%
    10.2}%
    \else%
      \def\HighMassEstimates@IV@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HighMassEstimates@IV@out
}\newcommand\HighMassEstimates@V[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HighMassEstimates@V@out{%
    \{%
      "median": 46.6,
      "5th percentile": 39.9,
      "95th percentile": 58.2,
      "error plus": 11.6,
      "error minus": 6.7%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HighMassEstimates@V@out{%
    46.6}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HighMassEstimates@V@out{%
    39.9}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HighMassEstimates@V@out{%
    58.2}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HighMassEstimates@V@out{%
    11.6}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HighMassEstimates@V@out{%
    6.7}%
    \else%
      \def\HighMassEstimates@V@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HighMassEstimates@V@out
}\newcommand\HighMassEstimates@VI[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HighMassEstimates@VI@out{%
    \{%
      "median": 0.6,
      "5th percentile": 0.2,
      "95th percentile": 0.9,
      "error plus": 0.3,
      "error minus": 0.5%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HighMassEstimates@VI@out{%
    0.6}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HighMassEstimates@VI@out{%
    0.2}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HighMassEstimates@VI@out{%
    0.9}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HighMassEstimates@VI@out{%
    0.3}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HighMassEstimates@VI@out{%
    0.5}%
    \else%
      \def\HighMassEstimates@VI@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HighMassEstimates@VI@out
}\newcommand\HighMassEstimates@VII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\HighMassEstimates@VII@out{%
    \{%
      "median": 45.5,
      "5th percentile": 40.4,
      "95th percentile": 52.4,
      "error plus": 6.9,
      "error minus": 5.2%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\HighMassEstimates@VII@out{%
    45.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\HighMassEstimates@VII@out{%
    40.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\HighMassEstimates@VII@out{%
    52.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\HighMassEstimates@VII@out{%
    6.9}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\HighMassEstimates@VII@out{%
    5.2}%
    \else%
      \def\HighMassEstimates@VII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \HighMassEstimates@VII@out
}%
\makeatother%
\makeatletter%
\newcommand\OverviewEstimates[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@out{%
    \{%
      "fullpop\_gap\_depth": \{%
        "99th percentile": 0.88%
      \},
      "bkpl2pk\_alpha\_1": \{%
        "median": 1.5,
        "5th percentile": 0.1,
        "95th percentile": 2.5,
        "error plus": 1.0,
        "error minus": 1.4%
      \},
      "bkpl2pk\_alpha\_2": \{%
        "median": 5.4,
        "5th percentile": 3.9,
        "95th percentile": 6.8,
        "error plus": 1.4,
        "error minus": 1.6%
      \},
      "alpha\_2\_steepness": 99.6,
      "break\_mass": \{%
        "median": 37.5,
        "5th percentile": 29.6,
        "95th percentile": 48.3,
        "error plus": 10.9,
        "error minus": 7.8%
      \},
      "beta\_q": \{%
        "median": 1.0,
        "5th percentile": 0.4,
        "95th percentile": 1.8,
        "error plus": 0.8,
        "error minus": 0.7%
      \},
      "pp\_10msun\_fracs": \{%
        "median": 60,
        "5th percentile": 51,
        "95th percentile": 68,
        "error plus": 8,
        "error minus": 10%
      \},
      "bkpl2pk\_10msun\_fracs": \{%
        "median": 72,
        "5th percentile": 63,
        "95th percentile": 79,
        "error plus": 7,
        "error minus": 9%
      \},
      "bkpl2pk\_aleq\_half\_fracs": \{%
        "median": 80,
        "5th percentile": 75,
        "95th percentile": 84,
        "error plus": 4,
        "error minus": 5%
      \},
      "pp\_aleq\_half\_fracs": \{%
        "median": 73,
        "5th percentile": 69,
        "95th percentile": 77,
        "error plus": 4,
        "error minus": 4%
      \},
      "pp\_aligned\_fracs": \{%
        "median": 57,
        "5th percentile": 52,
        "95th percentile": 62,
        "error plus": 5,
        "error minus": 5%
      \},
      "bkpl2pk\_aligned\_fracs": \{%
        "median": 54,
        "5th percentile": 50,
        "95th percentile": 60,
        "error plus": 6,
        "error minus": 4%
      \},
      "pp\_neg\_chieff\_frac": \{%
        "median": 36,
        "5th percentile": 30,
        "95th percentile": 42,
        "error plus": 6,
        "error minus": 6%
      \},
      "bsn\_neg\_chieff\_frac": \{%
        "median": 39,
        "5th percentile": 32,
        "95th percentile": 46,
        "error plus": 7,
        "error minus": 7%
      \},
      "bsn\_chieff\_asymmetry": \{%
        "median": 22,
        "5th percentile": 9,
        "95th percentile": 35,
        "error plus": 13,
        "error minus": 13%
      \},
      "pp\_chieff\_asymmetry": \{%
        "median": 28,
        "5th percentile": 17,
        "95th percentile": 40,
        "error plus": 11,
        "error minus": 12%
      \},
      "bsn\_chieff\_delchi": \{%
        "median": 0.22,
        "5th percentile": 0.09,
        "95th percentile": 0.35,
        "error plus": 0.13,
        "error minus": 0.13%
      \},
      "pp\_chieff\_delchi": \{%
        "median": 0.28,
        "5th percentile": 0.17,
        "95th percentile": 0.4,
        "error plus": 0.11,
        "error minus": 0.12%
      \},
      "bsn\_chieff\_skew": \{%
        "median": 0.38,
        "5th percentile": 0.13,
        "95th percentile": 0.68,
        "error plus": 0.3,
        "error minus": 0.25%
      \},
      "pp\_chieff\_skew": \{%
        "median": 0.02,
        "5th percentile": {-}0.25,
        "95th percentile": 0.28,
        "error plus": 0.26,
        "error minus": 0.27%
      \},
      "bsn\_chieff\_skew\_cred": 99.9,
      "pp\_bbh\_rates": \{%
        "median": 32.8,
        "5th percentile": 25.2,
        "95th percentile": 43.5,
        "error plus": 10.7,
        "error minus": 7.6%
      \},
      "bkpl2pk\_bbh\_rates": \{%
        "median": 30.4,
        "5th percentile": 25.0,
        "95th percentile": 36.9,
        "error plus": 6.5,
        "error minus": 5.4%
      \},
      "bbh\_rate\_uncertainity\_shrink": 20,
      "bkpl2pk\_kappa\_z": \{%
        "median": 2.5,
        "5th percentile": 1.8,
        "95th percentile": 3.2,
        "error plus": 0.7,
        "error minus": 0.7%
      \},
      "TGMM\_dominant\_mode\_fracs": \{%
        "median": 0.85,
        "5th percentile": 0.75,
        "95th percentile": 0.91,
        "error plus": 0.06,
        "error minus": 0.09%
      \},
      "TGMM\_subdominant\_mode\_fracs": \{%
        "median": 0.15,
        "5th percentile": 0.09,
        "95th percentile": 0.25,
        "error plus": 0.09,
        "error minus": 0.06%
      \},
      "MD\_BBH\_def\_log10\_bayes": {-}0.15%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{fullpop_gap_depth}=0%
      \let\OverviewEstimates@out\OverviewEstimates@I%
    \else%
      \ifnum\pdfstrcmp{#1}{bkpl2pk_alpha_1}=0%
      \let\OverviewEstimates@out\OverviewEstimates@II%
    \else%
      \ifnum\pdfstrcmp{#1}{bkpl2pk_alpha_2}=0%
      \let\OverviewEstimates@out\OverviewEstimates@III%
    \else%
      \ifnum\pdfstrcmp{#1}{alpha_2_steepness}=0%
      \def\OverviewEstimates@out{%
    99.6}%
    \else%
      \ifnum\pdfstrcmp{#1}{break_mass}=0%
      \let\OverviewEstimates@out\OverviewEstimates@IV%
    \else%
      \ifnum\pdfstrcmp{#1}{beta_q}=0%
      \let\OverviewEstimates@out\OverviewEstimates@V%
    \else%
      \ifnum\pdfstrcmp{#1}{pp_10msun_fracs}=0%
      \let\OverviewEstimates@out\OverviewEstimates@VI%
    \else%
      \ifnum\pdfstrcmp{#1}{bkpl2pk_10msun_fracs}=0%
      \let\OverviewEstimates@out\OverviewEstimates@VII%
    \else%
      \ifnum\pdfstrcmp{#1}{bkpl2pk_aleq_half_fracs}=0%
      \let\OverviewEstimates@out\OverviewEstimates@VIII%
    \else%
      \ifnum\pdfstrcmp{#1}{pp_aleq_half_fracs}=0%
      \let\OverviewEstimates@out\OverviewEstimates@IX%
    \else%
      \ifnum\pdfstrcmp{#1}{pp_aligned_fracs}=0%
      \let\OverviewEstimates@out\OverviewEstimates@X%
    \else%
      \ifnum\pdfstrcmp{#1}{bkpl2pk_aligned_fracs}=0%
      \let\OverviewEstimates@out\OverviewEstimates@XI%
    \else%
      \ifnum\pdfstrcmp{#1}{pp_neg_chieff_frac}=0%
      \let\OverviewEstimates@out\OverviewEstimates@XII%
    \else%
      \ifnum\pdfstrcmp{#1}{bsn_neg_chieff_frac}=0%
      \let\OverviewEstimates@out\OverviewEstimates@XIII%
    \else%
      \ifnum\pdfstrcmp{#1}{bsn_chieff_asymmetry}=0%
      \let\OverviewEstimates@out\OverviewEstimates@XIV%
    \else%
      \ifnum\pdfstrcmp{#1}{pp_chieff_asymmetry}=0%
      \let\OverviewEstimates@out\OverviewEstimates@XV%
    \else%
      \ifnum\pdfstrcmp{#1}{bsn_chieff_delchi}=0%
      \let\OverviewEstimates@out\OverviewEstimates@XVI%
    \else%
      \ifnum\pdfstrcmp{#1}{pp_chieff_delchi}=0%
      \let\OverviewEstimates@out\OverviewEstimates@XVII%
    \else%
      \ifnum\pdfstrcmp{#1}{bsn_chieff_skew}=0%
      \let\OverviewEstimates@out\OverviewEstimates@XVIII%
    \else%
      \ifnum\pdfstrcmp{#1}{pp_chieff_skew}=0%
      \let\OverviewEstimates@out\OverviewEstimates@XIX%
    \else%
      \ifnum\pdfstrcmp{#1}{bsn_chieff_skew_cred}=0%
      \def\OverviewEstimates@out{%
    99.9}%
    \else%
      \ifnum\pdfstrcmp{#1}{pp_bbh_rates}=0%
      \let\OverviewEstimates@out\OverviewEstimates@XX%
    \else%
      \ifnum\pdfstrcmp{#1}{bkpl2pk_bbh_rates}=0%
      \let\OverviewEstimates@out\OverviewEstimates@XXI%
    \else%
      \ifnum\pdfstrcmp{#1}{bbh_rate_uncertainity_shrink}=0%
      \def\OverviewEstimates@out{%
    20}%
    \else%
      \ifnum\pdfstrcmp{#1}{bkpl2pk_kappa_z}=0%
      \let\OverviewEstimates@out\OverviewEstimates@XXII%
    \else%
      \ifnum\pdfstrcmp{#1}{TGMM_dominant_mode_fracs}=0%
      \let\OverviewEstimates@out\OverviewEstimates@XXIII%
    \else%
      \ifnum\pdfstrcmp{#1}{TGMM_subdominant_mode_fracs}=0%
      \let\OverviewEstimates@out\OverviewEstimates@XXIV%
    \else%
      \ifnum\pdfstrcmp{#1}{MD_BBH_def_log10_bayes}=0%
      \def\OverviewEstimates@out{%
    {-}0.15}%
    \else%
      \def\OverviewEstimates@out{%
    ??}%
    \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@out
}\newcommand\OverviewEstimates@I[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@I@out{%
    \{%
      "99th percentile": 0.88%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{99th percentile}=0%
      \def\OverviewEstimates@I@out{%
    0.88}%
    \else%
      \def\OverviewEstimates@I@out{%
    ??}%
    \fi
  \fi
  \OverviewEstimates@I@out
}\newcommand\OverviewEstimates@II[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@II@out{%
    \{%
      "median": 1.5,
      "5th percentile": 0.1,
      "95th percentile": 2.5,
      "error plus": 1.0,
      "error minus": 1.4%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@II@out{%
    1.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@II@out{%
    0.1}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@II@out{%
    2.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@II@out{%
    1.0}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@II@out{%
    1.4}%
    \else%
      \def\OverviewEstimates@II@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@II@out
}\newcommand\OverviewEstimates@III[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@III@out{%
    \{%
      "median": 5.4,
      "5th percentile": 3.9,
      "95th percentile": 6.8,
      "error plus": 1.4,
      "error minus": 1.6%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@III@out{%
    5.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@III@out{%
    3.9}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@III@out{%
    6.8}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@III@out{%
    1.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@III@out{%
    1.6}%
    \else%
      \def\OverviewEstimates@III@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@III@out
}\newcommand\OverviewEstimates@IV[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@IV@out{%
    \{%
      "median": 37.5,
      "5th percentile": 29.6,
      "95th percentile": 48.3,
      "error plus": 10.9,
      "error minus": 7.8%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@IV@out{%
    37.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@IV@out{%
    29.6}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@IV@out{%
    48.3}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@IV@out{%
    10.9}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@IV@out{%
    7.8}%
    \else%
      \def\OverviewEstimates@IV@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@IV@out
}\newcommand\OverviewEstimates@V[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@V@out{%
    \{%
      "median": 1.0,
      "5th percentile": 0.4,
      "95th percentile": 1.8,
      "error plus": 0.8,
      "error minus": 0.7%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@V@out{%
    1.0}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@V@out{%
    0.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@V@out{%
    1.8}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@V@out{%
    0.8}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@V@out{%
    0.7}%
    \else%
      \def\OverviewEstimates@V@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@V@out
}\newcommand\OverviewEstimates@VI[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@VI@out{%
    \{%
      "median": 60,
      "5th percentile": 51,
      "95th percentile": 68,
      "error plus": 8,
      "error minus": 10%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@VI@out{%
    60}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@VI@out{%
    51}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@VI@out{%
    68}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@VI@out{%
    8}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@VI@out{%
    10}%
    \else%
      \def\OverviewEstimates@VI@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@VI@out
}\newcommand\OverviewEstimates@VII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@VII@out{%
    \{%
      "median": 72,
      "5th percentile": 63,
      "95th percentile": 79,
      "error plus": 7,
      "error minus": 9%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@VII@out{%
    72}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@VII@out{%
    63}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@VII@out{%
    79}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@VII@out{%
    7}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@VII@out{%
    9}%
    \else%
      \def\OverviewEstimates@VII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@VII@out
}\newcommand\OverviewEstimates@VIII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@VIII@out{%
    \{%
      "median": 80,
      "5th percentile": 75,
      "95th percentile": 84,
      "error plus": 4,
      "error minus": 5%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@VIII@out{%
    80}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@VIII@out{%
    75}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@VIII@out{%
    84}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@VIII@out{%
    4}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@VIII@out{%
    5}%
    \else%
      \def\OverviewEstimates@VIII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@VIII@out
}\newcommand\OverviewEstimates@IX[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@IX@out{%
    \{%
      "median": 73,
      "5th percentile": 69,
      "95th percentile": 77,
      "error plus": 4,
      "error minus": 4%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@IX@out{%
    73}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@IX@out{%
    69}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@IX@out{%
    77}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@IX@out{%
    4}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@IX@out{%
    4}%
    \else%
      \def\OverviewEstimates@IX@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@IX@out
}\newcommand\OverviewEstimates@X[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@X@out{%
    \{%
      "median": 57,
      "5th percentile": 52,
      "95th percentile": 62,
      "error plus": 5,
      "error minus": 5%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@X@out{%
    57}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@X@out{%
    52}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@X@out{%
    62}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@X@out{%
    5}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@X@out{%
    5}%
    \else%
      \def\OverviewEstimates@X@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@X@out
}\newcommand\OverviewEstimates@XI[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@XI@out{%
    \{%
      "median": 54,
      "5th percentile": 50,
      "95th percentile": 60,
      "error plus": 6,
      "error minus": 4%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@XI@out{%
    54}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@XI@out{%
    50}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@XI@out{%
    60}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@XI@out{%
    6}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@XI@out{%
    4}%
    \else%
      \def\OverviewEstimates@XI@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@XI@out
}\newcommand\OverviewEstimates@XII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@XII@out{%
    \{%
      "median": 36,
      "5th percentile": 30,
      "95th percentile": 42,
      "error plus": 6,
      "error minus": 6%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@XII@out{%
    36}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@XII@out{%
    30}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@XII@out{%
    42}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@XII@out{%
    6}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@XII@out{%
    6}%
    \else%
      \def\OverviewEstimates@XII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@XII@out
}\newcommand\OverviewEstimates@XIII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@XIII@out{%
    \{%
      "median": 39,
      "5th percentile": 32,
      "95th percentile": 46,
      "error plus": 7,
      "error minus": 7%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@XIII@out{%
    39}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@XIII@out{%
    32}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@XIII@out{%
    46}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@XIII@out{%
    7}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@XIII@out{%
    7}%
    \else%
      \def\OverviewEstimates@XIII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@XIII@out
}\newcommand\OverviewEstimates@XIV[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@XIV@out{%
    \{%
      "median": 22,
      "5th percentile": 9,
      "95th percentile": 35,
      "error plus": 13,
      "error minus": 13%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@XIV@out{%
    22}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@XIV@out{%
    9}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@XIV@out{%
    35}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@XIV@out{%
    13}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@XIV@out{%
    13}%
    \else%
      \def\OverviewEstimates@XIV@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@XIV@out
}\newcommand\OverviewEstimates@XV[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@XV@out{%
    \{%
      "median": 28,
      "5th percentile": 17,
      "95th percentile": 40,
      "error plus": 11,
      "error minus": 12%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@XV@out{%
    28}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@XV@out{%
    17}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@XV@out{%
    40}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@XV@out{%
    11}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@XV@out{%
    12}%
    \else%
      \def\OverviewEstimates@XV@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@XV@out
}\newcommand\OverviewEstimates@XVI[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@XVI@out{%
    \{%
      "median": 0.22,
      "5th percentile": 0.09,
      "95th percentile": 0.35,
      "error plus": 0.13,
      "error minus": 0.13%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@XVI@out{%
    0.22}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@XVI@out{%
    0.09}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@XVI@out{%
    0.35}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@XVI@out{%
    0.13}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@XVI@out{%
    0.13}%
    \else%
      \def\OverviewEstimates@XVI@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@XVI@out
}\newcommand\OverviewEstimates@XVII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@XVII@out{%
    \{%
      "median": 0.28,
      "5th percentile": 0.17,
      "95th percentile": 0.4,
      "error plus": 0.11,
      "error minus": 0.12%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@XVII@out{%
    0.28}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@XVII@out{%
    0.17}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@XVII@out{%
    0.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@XVII@out{%
    0.11}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@XVII@out{%
    0.12}%
    \else%
      \def\OverviewEstimates@XVII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@XVII@out
}\newcommand\OverviewEstimates@XVIII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@XVIII@out{%
    \{%
      "median": 0.38,
      "5th percentile": 0.13,
      "95th percentile": 0.68,
      "error plus": 0.3,
      "error minus": 0.25%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@XVIII@out{%
    0.38}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@XVIII@out{%
    0.13}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@XVIII@out{%
    0.68}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@XVIII@out{%
    0.3}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@XVIII@out{%
    0.25}%
    \else%
      \def\OverviewEstimates@XVIII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@XVIII@out
}\newcommand\OverviewEstimates@XIX[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@XIX@out{%
    \{%
      "median": 0.02,
      "5th percentile": {-}0.25,
      "95th percentile": 0.28,
      "error plus": 0.26,
      "error minus": 0.27%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@XIX@out{%
    0.02}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@XIX@out{%
    {-}0.25}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@XIX@out{%
    0.28}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@XIX@out{%
    0.26}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@XIX@out{%
    0.27}%
    \else%
      \def\OverviewEstimates@XIX@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@XIX@out
}\newcommand\OverviewEstimates@XX[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@XX@out{%
    \{%
      "median": 32.8,
      "5th percentile": 25.2,
      "95th percentile": 43.5,
      "error plus": 10.7,
      "error minus": 7.6%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@XX@out{%
    32.8}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@XX@out{%
    25.2}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@XX@out{%
    43.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@XX@out{%
    10.7}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@XX@out{%
    7.6}%
    \else%
      \def\OverviewEstimates@XX@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@XX@out
}\newcommand\OverviewEstimates@XXI[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@XXI@out{%
    \{%
      "median": 30.4,
      "5th percentile": 25.0,
      "95th percentile": 36.9,
      "error plus": 6.5,
      "error minus": 5.4%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@XXI@out{%
    30.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@XXI@out{%
    25.0}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@XXI@out{%
    36.9}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@XXI@out{%
    6.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@XXI@out{%
    5.4}%
    \else%
      \def\OverviewEstimates@XXI@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@XXI@out
}\newcommand\OverviewEstimates@XXII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@XXII@out{%
    \{%
      "median": 2.5,
      "5th percentile": 1.8,
      "95th percentile": 3.2,
      "error plus": 0.7,
      "error minus": 0.7%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@XXII@out{%
    2.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@XXII@out{%
    1.8}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@XXII@out{%
    3.2}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@XXII@out{%
    0.7}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@XXII@out{%
    0.7}%
    \else%
      \def\OverviewEstimates@XXII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@XXII@out
}\newcommand\OverviewEstimates@XXIII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@XXIII@out{%
    \{%
      "median": 0.85,
      "5th percentile": 0.75,
      "95th percentile": 0.91,
      "error plus": 0.06,
      "error minus": 0.09%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@XXIII@out{%
    0.85}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@XXIII@out{%
    0.75}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@XXIII@out{%
    0.91}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@XXIII@out{%
    0.06}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@XXIII@out{%
    0.09}%
    \else%
      \def\OverviewEstimates@XXIII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@XXIII@out
}\newcommand\OverviewEstimates@XXIV[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\OverviewEstimates@XXIV@out{%
    \{%
      "median": 0.15,
      "5th percentile": 0.09,
      "95th percentile": 0.25,
      "error plus": 0.09,
      "error minus": 0.06%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\OverviewEstimates@XXIV@out{%
    0.15}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\OverviewEstimates@XXIV@out{%
    0.09}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\OverviewEstimates@XXIV@out{%
    0.25}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\OverviewEstimates@XXIV@out{%
    0.09}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\OverviewEstimates@XXIV@out{%
    0.06}%
    \else%
      \def\OverviewEstimates@XXIV@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \OverviewEstimates@XXIV@out
}%
\makeatother%
\makeatletter%
\newcommand\RateEstimates[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\RateEstimates@out{%
    \{%
      "pp\_bns\_limits": \{%
        "median": 23.4,
        "5th percentile": 5.1,
        "95th percentile": 78.1,
        "error plus": 54.7,
        "error minus": 18.2%
      \},
      "pp\_nsbh\_limits": \{%
        "median": 15.9,
        "5th percentile": 7.1,
        "95th percentile": 32.8,
        "error plus": 16.9,
        "error minus": 8.9%
      \},
      "pp\_bbh\_limits": \{%
        "median": 24.3,
        "5th percentile": 19.0,
        "95th percentile": 30.8,
        "error plus": 6.6,
        "error minus": 5.2%
      \},
      "pp\_imbh\_limits": \{%
        "median": 2.5,
        "5th percentile": 0.4,
        "95th percentile": 12.8,
        "error plus": 10.3,
        "error minus": 2.1%
      \},
      "pp\_bbh\_z02\_limits": \{%
        "median": 37.5,
        "5th percentile": 28.4,
        "95th percentile": 49.4,
        "error plus": 11.9,
        "error minus": 9.1%
      \},
      "pp\_imbh\_z02\_limits": \{%
        "median": 3.8,
        "5th percentile": 0.6,
        "95th percentile": 19.9,
        "error plus": 16.1,
        "error minus": 3.3%
      \},
      "fp\_bns\_limits": \{%
        "median": 59.3,
        "5th percentile": 15.4,
        "95th percentile": 154.7,
        "error plus": 95.4,
        "error minus": 43.9%
      \},
      "fp\_nsbh\_limits": \{%
        "median": 14.2,
        "5th percentile": 6.7,
        "95th percentile": 26.3,
        "error plus": 12.0,
        "error minus": 7.5%
      \},
      "fp\_bbh\_limits": \{%
        "median": 22.7,
        "5th percentile": 18.0,
        "95th percentile": 28.7,
        "error plus": 6.0,
        "error minus": 4.7%
      \},
      "fp\_imbh\_limits": \{%
        "median": 4.0,
        "5th percentile": 0.6,
        "95th percentile": 14.4,
        "error plus": 10.4,
        "error minus": 3.4%
      \},
      "fp\_bbh\_z02\_limits": \{%
        "median": 36.0,
        "5th percentile": 27.5,
        "95th percentile": 47.1,
        "error plus": 11.1,
        "error minus": 8.5%
      \},
      "fp\_imbh\_z02\_limits": \{%
        "median": 6.4,
        "5th percentile": 1.0,
        "95th percentile": 23.1,
        "error plus": 16.7,
        "error minus": 5.3%
      \}%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{pp_bns_limits}=0%
      \let\RateEstimates@out\RateEstimates@I%
    \else%
      \ifnum\pdfstrcmp{#1}{pp_nsbh_limits}=0%
      \let\RateEstimates@out\RateEstimates@II%
    \else%
      \ifnum\pdfstrcmp{#1}{pp_bbh_limits}=0%
      \let\RateEstimates@out\RateEstimates@III%
    \else%
      \ifnum\pdfstrcmp{#1}{pp_imbh_limits}=0%
      \let\RateEstimates@out\RateEstimates@IV%
    \else%
      \ifnum\pdfstrcmp{#1}{pp_bbh_z02_limits}=0%
      \let\RateEstimates@out\RateEstimates@V%
    \else%
      \ifnum\pdfstrcmp{#1}{pp_imbh_z02_limits}=0%
      \let\RateEstimates@out\RateEstimates@VI%
    \else%
      \ifnum\pdfstrcmp{#1}{fp_bns_limits}=0%
      \let\RateEstimates@out\RateEstimates@VII%
    \else%
      \ifnum\pdfstrcmp{#1}{fp_nsbh_limits}=0%
      \let\RateEstimates@out\RateEstimates@VIII%
    \else%
      \ifnum\pdfstrcmp{#1}{fp_bbh_limits}=0%
      \let\RateEstimates@out\RateEstimates@IX%
    \else%
      \ifnum\pdfstrcmp{#1}{fp_imbh_limits}=0%
      \let\RateEstimates@out\RateEstimates@X%
    \else%
      \ifnum\pdfstrcmp{#1}{fp_bbh_z02_limits}=0%
      \let\RateEstimates@out\RateEstimates@XI%
    \else%
      \ifnum\pdfstrcmp{#1}{fp_imbh_z02_limits}=0%
      \let\RateEstimates@out\RateEstimates@XII%
    \else%
      \def\RateEstimates@out{%
    ??}%
    \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
  \fi
  \RateEstimates@out
}\newcommand\RateEstimates@I[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\RateEstimates@I@out{%
    \{%
      "median": 23.4,
      "5th percentile": 5.1,
      "95th percentile": 78.1,
      "error plus": 54.7,
      "error minus": 18.2%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\RateEstimates@I@out{%
    23.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\RateEstimates@I@out{%
    5.1}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\RateEstimates@I@out{%
    78.1}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\RateEstimates@I@out{%
    54.7}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\RateEstimates@I@out{%
    18.2}%
    \else%
      \def\RateEstimates@I@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \RateEstimates@I@out
}\newcommand\RateEstimates@II[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\RateEstimates@II@out{%
    \{%
      "median": 15.9,
      "5th percentile": 7.1,
      "95th percentile": 32.8,
      "error plus": 16.9,
      "error minus": 8.9%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\RateEstimates@II@out{%
    15.9}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\RateEstimates@II@out{%
    7.1}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\RateEstimates@II@out{%
    32.8}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\RateEstimates@II@out{%
    16.9}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\RateEstimates@II@out{%
    8.9}%
    \else%
      \def\RateEstimates@II@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \RateEstimates@II@out
}\newcommand\RateEstimates@III[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\RateEstimates@III@out{%
    \{%
      "median": 24.3,
      "5th percentile": 19.0,
      "95th percentile": 30.8,
      "error plus": 6.6,
      "error minus": 5.2%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\RateEstimates@III@out{%
    24.3}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\RateEstimates@III@out{%
    19.0}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\RateEstimates@III@out{%
    30.8}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\RateEstimates@III@out{%
    6.6}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\RateEstimates@III@out{%
    5.2}%
    \else%
      \def\RateEstimates@III@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \RateEstimates@III@out
}\newcommand\RateEstimates@IV[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\RateEstimates@IV@out{%
    \{%
      "median": 2.5,
      "5th percentile": 0.4,
      "95th percentile": 12.8,
      "error plus": 10.3,
      "error minus": 2.1%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\RateEstimates@IV@out{%
    2.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\RateEstimates@IV@out{%
    0.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\RateEstimates@IV@out{%
    12.8}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\RateEstimates@IV@out{%
    10.3}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\RateEstimates@IV@out{%
    2.1}%
    \else%
      \def\RateEstimates@IV@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \RateEstimates@IV@out
}\newcommand\RateEstimates@V[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\RateEstimates@V@out{%
    \{%
      "median": 37.5,
      "5th percentile": 28.4,
      "95th percentile": 49.4,
      "error plus": 11.9,
      "error minus": 9.1%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\RateEstimates@V@out{%
    37.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\RateEstimates@V@out{%
    28.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\RateEstimates@V@out{%
    49.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\RateEstimates@V@out{%
    11.9}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\RateEstimates@V@out{%
    9.1}%
    \else%
      \def\RateEstimates@V@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \RateEstimates@V@out
}\newcommand\RateEstimates@VI[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\RateEstimates@VI@out{%
    \{%
      "median": 3.8,
      "5th percentile": 0.6,
      "95th percentile": 19.9,
      "error plus": 16.1,
      "error minus": 3.3%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\RateEstimates@VI@out{%
    3.8}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\RateEstimates@VI@out{%
    0.6}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\RateEstimates@VI@out{%
    19.9}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\RateEstimates@VI@out{%
    16.1}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\RateEstimates@VI@out{%
    3.3}%
    \else%
      \def\RateEstimates@VI@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \RateEstimates@VI@out
}\newcommand\RateEstimates@VII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\RateEstimates@VII@out{%
    \{%
      "median": 59.3,
      "5th percentile": 15.4,
      "95th percentile": 154.7,
      "error plus": 95.4,
      "error minus": 43.9%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\RateEstimates@VII@out{%
    59.3}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\RateEstimates@VII@out{%
    15.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\RateEstimates@VII@out{%
    154.7}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\RateEstimates@VII@out{%
    95.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\RateEstimates@VII@out{%
    43.9}%
    \else%
      \def\RateEstimates@VII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \RateEstimates@VII@out
}\newcommand\RateEstimates@VIII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\RateEstimates@VIII@out{%
    \{%
      "median": 14.2,
      "5th percentile": 6.7,
      "95th percentile": 26.3,
      "error plus": 12.0,
      "error minus": 7.5%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\RateEstimates@VIII@out{%
    14.2}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\RateEstimates@VIII@out{%
    6.7}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\RateEstimates@VIII@out{%
    26.3}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\RateEstimates@VIII@out{%
    12.0}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\RateEstimates@VIII@out{%
    7.5}%
    \else%
      \def\RateEstimates@VIII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \RateEstimates@VIII@out
}\newcommand\RateEstimates@IX[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\RateEstimates@IX@out{%
    \{%
      "median": 22.7,
      "5th percentile": 18.0,
      "95th percentile": 28.7,
      "error plus": 6.0,
      "error minus": 4.7%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\RateEstimates@IX@out{%
    22.7}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\RateEstimates@IX@out{%
    18.0}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\RateEstimates@IX@out{%
    28.7}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\RateEstimates@IX@out{%
    6.0}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\RateEstimates@IX@out{%
    4.7}%
    \else%
      \def\RateEstimates@IX@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \RateEstimates@IX@out
}\newcommand\RateEstimates@X[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\RateEstimates@X@out{%
    \{%
      "median": 4.0,
      "5th percentile": 0.6,
      "95th percentile": 14.4,
      "error plus": 10.4,
      "error minus": 3.4%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\RateEstimates@X@out{%
    4.0}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\RateEstimates@X@out{%
    0.6}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\RateEstimates@X@out{%
    14.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\RateEstimates@X@out{%
    10.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\RateEstimates@X@out{%
    3.4}%
    \else%
      \def\RateEstimates@X@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \RateEstimates@X@out
}\newcommand\RateEstimates@XI[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\RateEstimates@XI@out{%
    \{%
      "median": 36.0,
      "5th percentile": 27.5,
      "95th percentile": 47.1,
      "error plus": 11.1,
      "error minus": 8.5%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\RateEstimates@XI@out{%
    36.0}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\RateEstimates@XI@out{%
    27.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\RateEstimates@XI@out{%
    47.1}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\RateEstimates@XI@out{%
    11.1}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\RateEstimates@XI@out{%
    8.5}%
    \else%
      \def\RateEstimates@XI@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \RateEstimates@XI@out
}\newcommand\RateEstimates@XII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\RateEstimates@XII@out{%
    \{%
      "median": 6.4,
      "5th percentile": 1.0,
      "95th percentile": 23.1,
      "error plus": 16.7,
      "error minus": 5.3%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\RateEstimates@XII@out{%
    6.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\RateEstimates@XII@out{%
    1.0}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\RateEstimates@XII@out{%
    23.1}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\RateEstimates@XII@out{%
    16.7}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\RateEstimates@XII@out{%
    5.3}%
    \else%
      \def\RateEstimates@XII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \RateEstimates@XII@out
}%
\makeatother%
\makeatletter%
\newcommand\SamplePurity[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\SamplePurity@out{%
    \{%
      "totalNumEvents": 267,
      "expectedNumFalseTrialsFactor": \{%
        "full": 9.56757117144523,
        "rounded": 9.6%
      \},
      "expectedNumFalseSimple": \{%
        "full": 2.621892792861307,
        "rounded": 2.6%
      \},
      "percentFalseTrialsFactor": \{%
        "full": 3.58335998930533,
        "rounded": 3.58%
      \},
      "percentFalseSimple": \{%
        "full": 0.9819823194237106,
        "rounded": 0.98%
      \},
      "totalAnalysisTimeYears": \{%
        "full": 1.9103253732856744,
        "rounded": 1.91%
      \}%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{totalNumEvents}=0%
      \def\SamplePurity@out{%
    267}%
    \else%
      \ifnum\pdfstrcmp{#1}{expectedNumFalseTrialsFactor}=0%
      \let\SamplePurity@out\SamplePurity@I%
    \else%
      \ifnum\pdfstrcmp{#1}{expectedNumFalseSimple}=0%
      \let\SamplePurity@out\SamplePurity@II%
    \else%
      \ifnum\pdfstrcmp{#1}{percentFalseTrialsFactor}=0%
      \let\SamplePurity@out\SamplePurity@III%
    \else%
      \ifnum\pdfstrcmp{#1}{percentFalseSimple}=0%
      \let\SamplePurity@out\SamplePurity@IV%
    \else%
      \ifnum\pdfstrcmp{#1}{totalAnalysisTimeYears}=0%
      \let\SamplePurity@out\SamplePurity@V%
    \else%
      \def\SamplePurity@out{%
    ??}%
    \fi\fi\fi\fi\fi\fi
  \fi
  \SamplePurity@out
}\newcommand\SamplePurity@I[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\SamplePurity@I@out{%
    \{%
      "full": 9.56757117144523,
      "rounded": 9.6%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{full}=0%
      \def\SamplePurity@I@out{%
    9.56757117144523}%
    \else%
      \ifnum\pdfstrcmp{#1}{rounded}=0%
      \def\SamplePurity@I@out{%
    9.6}%
    \else%
      \def\SamplePurity@I@out{%
    ??}%
    \fi\fi
  \fi
  \SamplePurity@I@out
}\newcommand\SamplePurity@II[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\SamplePurity@II@out{%
    \{%
      "full": 2.621892792861307,
      "rounded": 2.6%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{full}=0%
      \def\SamplePurity@II@out{%
    2.621892792861307}%
    \else%
      \ifnum\pdfstrcmp{#1}{rounded}=0%
      \def\SamplePurity@II@out{%
    2.6}%
    \else%
      \def\SamplePurity@II@out{%
    ??}%
    \fi\fi
  \fi
  \SamplePurity@II@out
}\newcommand\SamplePurity@III[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\SamplePurity@III@out{%
    \{%
      "full": 3.58335998930533,
      "rounded": 3.58%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{full}=0%
      \def\SamplePurity@III@out{%
    3.58335998930533}%
    \else%
      \ifnum\pdfstrcmp{#1}{rounded}=0%
      \def\SamplePurity@III@out{%
    3.58}%
    \else%
      \def\SamplePurity@III@out{%
    ??}%
    \fi\fi
  \fi
  \SamplePurity@III@out
}\newcommand\SamplePurity@IV[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\SamplePurity@IV@out{%
    \{%
      "full": 0.9819823194237106,
      "rounded": 0.98%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{full}=0%
      \def\SamplePurity@IV@out{%
    0.9819823194237106}%
    \else%
      \ifnum\pdfstrcmp{#1}{rounded}=0%
      \def\SamplePurity@IV@out{%
    0.98}%
    \else%
      \def\SamplePurity@IV@out{%
    ??}%
    \fi\fi
  \fi
  \SamplePurity@IV@out
}\newcommand\SamplePurity@V[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\SamplePurity@V@out{%
    \{%
      "full": 1.9103253732856744,
      "rounded": 1.91%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{full}=0%
      \def\SamplePurity@V@out{%
    1.9103253732856744}%
    \else%
      \ifnum\pdfstrcmp{#1}{rounded}=0%
      \def\SamplePurity@V@out{%
    1.91}%
    \else%
      \def\SamplePurity@V@out{%
    ??}%
    \fi\fi
  \fi
  \SamplePurity@V@out
}%
\makeatother%
\makeatletter%
\newcommand\test[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\test@out{%
    \{\}}%
  \else%
    \def\test@out{%
    ??}%
    
  \fi
  \test@out
}%
\makeatother%
\makeatletter%
\newcommand\thirtyfive[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\thirtyfive@out{%
    \{%
      "m1\_peak\_25\_40": \{%
        "median": 29.0,
        "5th percentile": 25.5,
        "95th percentile": 34.3,
        "error plus": 5.3,
        "error minus": 3.4%
      \},
      "m2\_peak\_25\_40": \{%
        "median": 27.8,
        "5th percentile": 25.5,
        "95th percentile": 31.5,
        "error plus": 3.7,
        "error minus": 2.2%
      \},
      "m1\_rate\_ratio\_30\_over\_25": \{%
        "median": 0.8,
        "5th percentile": 0.5,
        "95th percentile": 1.5,
        "error plus": 0.7,
        "error minus": 0.4%
      \},
      "m1\_rate\_ratio\_30\_over\_40": \{%
        "median": 2.2,
        "5th percentile": 1.3,
        "95th percentile": 3.8,
        "error plus": 1.6,
        "error minus": 1.0%
      \},
      "m2\_rate\_ratio\_30\_over\_25": \{%
        "median": 1.0,
        "5th percentile": 0.5,
        "95th percentile": 2.1,
        "error plus": 1.1,
        "error minus": 0.5%
      \},
      "m2\_rate\_ratio\_30\_over\_40": \{%
        "median": 7.9,
        "5th percentile": 3.6,
        "95th percentile": 17.4,
        "error plus": 9.4,
        "error minus": 4.4%
      \},
      "m2\_over\_m1\_decline\_30\_40\_factor": \{%
        "median": 3.5,
        "5th percentile": 1.4,
        "95th percentile": 8.7,
        "error plus": 5.1,
        "error minus": 2.1%
      \},
      "pp\_q\_rate\_ratio\_1\_over\_0p7": \{%
        "median": 1.9,
        "5th percentile": 0.5,
        "95th percentile": 6.7,
        "error plus": 4.8,
        "error minus": 1.4%
      \}%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{m1_peak_25_40}=0%
      \let\thirtyfive@out\thirtyfive@I%
    \else%
      \ifnum\pdfstrcmp{#1}{m2_peak_25_40}=0%
      \let\thirtyfive@out\thirtyfive@II%
    \else%
      \ifnum\pdfstrcmp{#1}{m1_rate_ratio_30_over_25}=0%
      \let\thirtyfive@out\thirtyfive@III%
    \else%
      \ifnum\pdfstrcmp{#1}{m1_rate_ratio_30_over_40}=0%
      \let\thirtyfive@out\thirtyfive@IV%
    \else%
      \ifnum\pdfstrcmp{#1}{m2_rate_ratio_30_over_25}=0%
      \let\thirtyfive@out\thirtyfive@V%
    \else%
      \ifnum\pdfstrcmp{#1}{m2_rate_ratio_30_over_40}=0%
      \let\thirtyfive@out\thirtyfive@VI%
    \else%
      \ifnum\pdfstrcmp{#1}{m2_over_m1_decline_30_40_factor}=0%
      \let\thirtyfive@out\thirtyfive@VII%
    \else%
      \ifnum\pdfstrcmp{#1}{pp_q_rate_ratio_1_over_0p7}=0%
      \let\thirtyfive@out\thirtyfive@VIII%
    \else%
      \def\thirtyfive@out{%
    ??}%
    \fi\fi\fi\fi\fi\fi\fi\fi
  \fi
  \thirtyfive@out
}\newcommand\thirtyfive@I[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\thirtyfive@I@out{%
    \{%
      "median": 29.0,
      "5th percentile": 25.5,
      "95th percentile": 34.3,
      "error plus": 5.3,
      "error minus": 3.4%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\thirtyfive@I@out{%
    29.0}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\thirtyfive@I@out{%
    25.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\thirtyfive@I@out{%
    34.3}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\thirtyfive@I@out{%
    5.3}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\thirtyfive@I@out{%
    3.4}%
    \else%
      \def\thirtyfive@I@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \thirtyfive@I@out
}\newcommand\thirtyfive@II[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\thirtyfive@II@out{%
    \{%
      "median": 27.8,
      "5th percentile": 25.5,
      "95th percentile": 31.5,
      "error plus": 3.7,
      "error minus": 2.2%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\thirtyfive@II@out{%
    27.8}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\thirtyfive@II@out{%
    25.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\thirtyfive@II@out{%
    31.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\thirtyfive@II@out{%
    3.7}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\thirtyfive@II@out{%
    2.2}%
    \else%
      \def\thirtyfive@II@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \thirtyfive@II@out
}\newcommand\thirtyfive@III[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\thirtyfive@III@out{%
    \{%
      "median": 0.8,
      "5th percentile": 0.5,
      "95th percentile": 1.5,
      "error plus": 0.7,
      "error minus": 0.4%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\thirtyfive@III@out{%
    0.8}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\thirtyfive@III@out{%
    0.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\thirtyfive@III@out{%
    1.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\thirtyfive@III@out{%
    0.7}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\thirtyfive@III@out{%
    0.4}%
    \else%
      \def\thirtyfive@III@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \thirtyfive@III@out
}\newcommand\thirtyfive@IV[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\thirtyfive@IV@out{%
    \{%
      "median": 2.2,
      "5th percentile": 1.3,
      "95th percentile": 3.8,
      "error plus": 1.6,
      "error minus": 1.0%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\thirtyfive@IV@out{%
    2.2}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\thirtyfive@IV@out{%
    1.3}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\thirtyfive@IV@out{%
    3.8}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\thirtyfive@IV@out{%
    1.6}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\thirtyfive@IV@out{%
    1.0}%
    \else%
      \def\thirtyfive@IV@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \thirtyfive@IV@out
}\newcommand\thirtyfive@V[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\thirtyfive@V@out{%
    \{%
      "median": 1.0,
      "5th percentile": 0.5,
      "95th percentile": 2.1,
      "error plus": 1.1,
      "error minus": 0.5%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\thirtyfive@V@out{%
    1.0}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\thirtyfive@V@out{%
    0.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\thirtyfive@V@out{%
    2.1}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\thirtyfive@V@out{%
    1.1}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\thirtyfive@V@out{%
    0.5}%
    \else%
      \def\thirtyfive@V@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \thirtyfive@V@out
}\newcommand\thirtyfive@VI[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\thirtyfive@VI@out{%
    \{%
      "median": 7.9,
      "5th percentile": 3.6,
      "95th percentile": 17.4,
      "error plus": 9.4,
      "error minus": 4.4%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\thirtyfive@VI@out{%
    7.9}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\thirtyfive@VI@out{%
    3.6}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\thirtyfive@VI@out{%
    17.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\thirtyfive@VI@out{%
    9.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\thirtyfive@VI@out{%
    4.4}%
    \else%
      \def\thirtyfive@VI@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \thirtyfive@VI@out
}\newcommand\thirtyfive@VII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\thirtyfive@VII@out{%
    \{%
      "median": 3.5,
      "5th percentile": 1.4,
      "95th percentile": 8.7,
      "error plus": 5.1,
      "error minus": 2.1%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\thirtyfive@VII@out{%
    3.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\thirtyfive@VII@out{%
    1.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\thirtyfive@VII@out{%
    8.7}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\thirtyfive@VII@out{%
    5.1}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\thirtyfive@VII@out{%
    2.1}%
    \else%
      \def\thirtyfive@VII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \thirtyfive@VII@out
}\newcommand\thirtyfive@VIII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\thirtyfive@VIII@out{%
    \{%
      "median": 1.9,
      "5th percentile": 0.5,
      "95th percentile": 6.7,
      "error plus": 4.8,
      "error minus": 1.4%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\thirtyfive@VIII@out{%
    1.9}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\thirtyfive@VIII@out{%
    0.5}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\thirtyfive@VIII@out{%
    6.7}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\thirtyfive@VIII@out{%
    4.8}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\thirtyfive@VIII@out{%
    1.4}%
    \else%
      \def\thirtyfive@VIII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \thirtyfive@VIII@out
}%
\makeatother%

